LRD-MPC: Efficient MPC Inference through Low-rank Decomposition

Secure Multi-party Computation (MPC) enables untrusted parties to jointly compute a function without revealing their inputs. Its application to machine learning (ML) has gained significant attention, particularly for secure inference services deployed across multiple cloud virtual machines (VMs), where each VM acts as an MPC party. Model providers secret-share model weights, and users secret-share inputs, ensuring that each server operates only on random shares. While MPC provides strong cryptographic guarantees, it incurs substantial computational and communication overhead. Deep neural networks rely heavily on convolutional and fully connected layers, which require costly matrix multiplications in MPC. To reduce this cost, we propose leveraging low-rank decomposition (LRD) for linear layers, replacing one large matrix multiplication with two smaller ones. Each matrix multiplication in MPC incurs a round of communication, meaning decomposing one matrix multiplication into two leads to an additional communication round. Second, the added matrix multiplication requires an additional truncation step to maintain numerical precision. Since truncation itself requires communication and computation, these overheads can offset the gains from decomposition. To address this, we introduce two complementary optimizations: truncation skipping and efficient linear layer concatenation. Truncation skipping removes the extra truncation induced by LRD, while linear layer concatenation pipelines operations to hide the additional communication round. Together, these techniques mitigate the main overheads of LRD in MPC and improve overall efficiency. Our approach is broadly applicable across MPC protocols. Experiments show up to 25% speedup in n-PC and 33% in 3-PC protocols over full-rank baselines, along with up to 52% GPU energy savings and 88% reduction in offline-phase latency.

==> tables/environment.tex <==

\begin{table}
    \centering
    \caption{Evaluation environments}
    \begin{tabular}{|c|c|} \hline
        CPU & AMD EPYC 7502 \\ \hline
        GPU &  Nvidia Quadro RTX 5000 \\ \hline
        DRAM & 512GB DDR4 \\ \hline
        vRAM & 16GB HBM \\ \hline
        OS & Ubuntu 20.04.6\\ \hline
        Kernel & Linux 5.4.0-162-generic \\ \hline
    \end{tabular}
    \label{tab:environ}
\end{table}

==> tables/motivation-power.tex <==
\begin{table}[h]
    \centering
    \caption{Linear layer power consumption (\%) in MPC inference online phase (5Gbps WAN)}
    \begin{tabular}{cc}
        \toprule
        \textbf{Protocol} &  \pc{n}    \\
        \midrule
        VGG   &  72.4\% \\
        \midrule
        BERT\textsubscript{\scriptsize LARGE}  & 67.8\% \\
        \midrule
        GCN & 85.3\% \\
        \bottomrule
    \end{tabular}
    \label{tab:motivation-power}
\end{table}

==> tables/offline_beaverTriple.tex <==

\begin{table}[h]
    \centering
    \caption{Reduction in Beaver triples needed to be generated for \pc{n} using \name{}}
    \begin{tabular}{cc}
        \toprule
         \textbf{Model} & \textbf{Reduction} \\
        \midrule
        WideResNet18 & 37.25\% \\
        \midrule
        VGG19 & 17.16\% \\
        \midrule
        GCN & 55.98\%\\
        \midrule BERT\textsubscript{\scriptsize LARGE} & 55.29\% \\
        \bottomrule
    \end{tabular}
    \label{tab:offline_beaver}
\end{table}

==> tables/pipe3-flow1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/3matmul-pipe1.pdf}
    \caption{Trio online phase matrix multiplication computation and communication workflow with efficient layer concatenation.}
    \label{fig:trio-flow-pipe}
\end{figure}
